Information-theoretic lower bounds on the oracle complexity of stochastic convex optimization

Relative to the large literature on upper bounds on complexity of convex optimization, lesser attention has been paid to the fundamental hardness of these problems. Given the extensive use of convex optimization in machine learning and statistics, gaining an understanding of these complexity-theoretic issues is important. In this paper, we study the complexity of stochastic convex optimization in an oracle model of computation. We improve upon known results and obtain tight minimax complexity estimates for various function classes.

==> macros.tex <==
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\fb}{\ensuremath{\bar{f}}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\renewcommand{\P}{\ensuremath{\mathbb{P}}}
\newcommand{\x}[1]{\ensuremath{x(#1)}}
\newcommand{\KL}{\ensuremath{\mbox{KL}}}
\newcommand{\conv}{\ensuremath{\varrho}}
\newcommand{\conveps}{\ensuremath{\varepsilon}}
\newcommand{\toss}{\ensuremath{b}}
\newcommand{\parama}{\ensuremath{\alpha}}
\newcommand{\paramb}{\ensuremath{\beta}}
\newcommand{\noisev}{\ensuremath{\nu}}
\newcommand{\noiseg}{\ensuremath{\bar{\nu}}}
\newcommand{\set}{\ensuremath{S}}
\newcommand{\meth}{\ensuremath{\mathcal{M}}}
\newcommand{\info}{\ensuremath{\phi}}
\renewcommand{\O}{\ensuremath{\mathcal{O}}}
\newcommand{\acc}{\ensuremath{\epsilon}}
\newcommand{\bestacc}{\epsilon^*}
\newcommand{\err}{\ensuremath{\delta}}
\renewcommand{\dim}{\ensuremath{d}}
\newcommand{\inrad}{\ensuremath{r}}
\newcommand{\disc}{\ensuremath{\rho}}
\newcommand{\errfun}{\ensuremath{\psi}}
\newcommand{\esta}[1]{\ensuremath{\widehat{\parama}(#1)}}
\newcommand{\estb}[1]{\ensuremath{\widehat{\paramb}(#1)}}
\newcommand{\fp}{\ensuremath{f^+}}
\newcommand{\fn}{\ensuremath{f^-}}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\lr}[3]{\ensuremath{\left #1 #2 \right #3}}
\newcommand{\coins}{\ensuremath{\Theta}}
\newcommand{\coin}{\ensuremath{\theta}}
\renewcommand{\show}{\ensuremath{\nu}}
\newcommand{\tot}{\ensuremath{N}}
\newcommand{\perm}{\ensuremath{\xi}}
\renewcommand{\it}{\ensuremath{i_t}}
\newcommand{\packset}{\ensuremath{\mathcal{V}}}
\newcommand{\packfrac}{\ensuremath{\tau}}
\newcommand{\indicator}{\ensuremath{\mathbb{I}}}
\newcommand{\e}{\ensuremath{\mbox{e}}}
\newcommand{\truth}{\ensuremath{\phi}}
\newcommand{\outrad}{\ensuremath{R}}
\newcommand{\oraclev}{\ensuremath{\widehat{f}}}
\newcommand{\oracleg}{\ensuremath{\widehat{g}}}
\newcommand{\sign}{\ensuremath{\mbox{sign}}}
\newcommand{\noise}{\ensuremath{\nu}}
\newcommand{\lipexp}{\ensuremath{p}}
\newcommand{\lipexpdual}{\ensuremath{q}}
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\ind}{\ensuremath{\mathbb{I}}}
\def\elem{x}
\def\fun{f}
\def\ConvSet{\set}
\def\FunSet{\mathcal{F}}
\def\InfoSet{\mathcal{I}}
\def\real{\mathbb{R}}

\def\accexp{\acc^{*}}
\def\methset{\mathbb{M}}
\def\defn{:=}
\def\funclassset{\mathcal{G}_{\operatorname{base}}}
\def\asphericity{\ensuremath{\rho}}
\def\prox{\Phi}
\def\norm#1{\|#1\|}
\def\dnorm#1{\|#1\|_*}
\newcommand{\Fstrong}{\ensuremath{\mathcal{F}_{\operatorname{\scriptsize{scv}}}}}
\newcommand{\Fsparse}{\ensuremath{\mathcal{F}_{\operatorname{\scriptsize{sp}}}}}
\newcommand{\Fconv}{\ensuremath{\mathcal{F}_{\operatorname{\scriptsize{cv}}}}}

